An Overview of Attacks and Defences on Intelligent Connected Vehicles

Cyber security is one of the most significant challenges in connected vehicular systems and connected vehicles are prone to different cybersecurity attacks that endanger passengers' safety. Cyber security in intelligent connected vehicles is composed of in-vehicle security and security of inter-vehicle communications. Security of Electronic Control Units (ECUs) and the Control Area Network (CAN) bus are the most significant parts of in-vehicle security. Besides, with the development of 4G LTE and 5G remote communication technologies for vehicle-toeverything (V2X) communications, the security of inter-vehicle communications is another potential problem. After giving a short introduction to the architecture of next-generation vehicles including driverless and intelligent vehicles, this review paper identifies a few major security attacks on the intelligent connected vehicles. Based on these attacks, we provide a comprehensive survey of available defences against these attacks and classify them into four categories, i.e. cryptography, network security, software vulnerability detection, and malware detection. We also explore the future directions for preventing attacks on intelligent vehicle systems.

==> sec_method.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Research Method}
\label{sec:method}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section studies the existing research efforts that contribute to the research topics on securing modern vehicle systems. 
We conducted a \emph{systematic literature review} following the guidelines proposed by Webster and Watson~\cite{Kitchenham07guidelinesfor, Webster02, Brocke09}.
As a result, our literature review process consists of three main phases: literature search and collection, literature selection, and literature analysis and evaluation. 
A detailed documentation of this review process is also provided in this section. 
To keep the process manageable with limited resources, instead of conducting a truly exhaustive literature review across various domains, we aim for a generous coverage of representative samples of the research work on and closely related to the topic of securing modern vehicles from the perspective of autonomous vehicle manufacturers.\footnote{We classify the coverage of our literature review to be ‘representative’ according to Cooper’s taxonomy~\cite{Cooper88}.}
%
%Table \ref{tab:table1} - Research questions:
%The first research question should answer the following aspects:
%\begin{itemize}
%  \item The relationships between SOA and microservices \cite{Zimmermann2017}
%  \item How do you see the relationship between REST and
%microservices? 
%\item Is the usage of Web protocols required
%and sufficient? 
%\item Is RESTful HTTP only one of several valid remote communication options in the microservices architect’s toolbox and, if so, what are the decision drivers
%when choosing an option? \cite{Zimmermann2017}
%\item What are the benefits of adopting microservices architecture?
%\end{itemize}
%
%The second research question should answer the following aspects:
%\begin{itemize}
%  \item In which business domain and socio-technical context
%(or application genre and software operating range w.r.t.
%quality attributes) have you applied microservices
%concepts and technologies—either successfully or unsuc-
%cessfully? \cite{Zimmermann2017}
%  \item Which microservices principles (e.g., “independently
%deployable services”) did you use in your microser-
%vices architecture designs, and how did you implement
%them (patterns, frameworks, middleware, tools)? Did you
%deploy to public or private cloud offerings (e.g. Amazon
%Lambdas, Google Cloud Function) or to more traditional
%application hosting environments? \cite{Zimmermann2017}
%\item Which research and development challenges for a broad
%and sustainable adoption of microservices can the
%service-oriented computing community derive from your
%experience?  \cite{Zimmermann2017}
%\item \cite{Zimmermann2017} states that "the enterprise service
%bus (ESB) pattern [33], its commercial implementations and
%their project use have been criticized by members of the
%microservices community as overly heavyweight, inflexible
%and unmanageable; however, the requirement for such inte-
%gration capabilities cannot simply be argued away. Hence,
%message routing and transformation patterns [9] have to
%be supported and possibly adapted to fit the microservices
%tenets: Do emerging microservices patterns such as C. Robin-
%son’s “API Gateway” \footnote{https://www.infoq.com/articles/microservices-intro} provide sufficient design guidance
%or are additional ones needed? If so, how to stitch such pat-
%terns together? Should transformations be wrapped in and
%deployed as first-class microservices (of a particular type)?"
%\end{itemize}
%
%The third research question should answer the following aspects:
%\begin{itemize}
%  \item "How did you find an adequate/a suited service cut (e.g.,
%how small/fine is small/fine enough)? How can DDD \cite{evans2003domain} (and/or other approaches to application scoping and
%functional partitioning) be applied to decompose mono-
%liths into services—practitioners have reported that they
%would welcome guidance that is more concrete than the
%rather frequently stated advice “define a bounded context
%for each domain concept to be exposed as service”?" \cite{Zimmermann2017}
%  \item How do we ensure end-to-end data integrity in microservices architectures, either centrally or de-centrally?
%  \item Do you have any advice/guidance how to compose
%microservices into end user client applications? How
%about application-level intermediaries, i.e., can microser-
%vices also be clients of other microservices? If so,
%how to avoid microservice deployment dependency and
%dynamic invocation “spaghetti” (e.g., cycles, overly deep
%invocation chains)? Do you see a need for/can you rec-
%ommend any tools, libraries, frameworks, middleware
%that can assist with this task, or is plain old development
%(applying state-of-the-art software engineering practices)
%sufficient? \cite{Zimmermann2017}
%\item Can you report on your technical and organizational
%scaling strategies (e.g., when having to deal with large
%services landscapes and rich/complex domain models
%with hundreds or thousands of interconnected entities)?
%Which tactics and patterns support these strategies well? \cite{Zimmermann2017}
%\item Did you define machine-readable service contracts?
%If so, what should they cover and how should they
%be expressed (e.g., are all REST maturity required,
%including support for Hypertext as the Engine of
%Application State (HATEOAS), is billing infor-
%mation included)? If not, how did you achieve syn-
%tactic and semantic interoperability between service
%consumers and providers? \cite{Zimmermann2017}
%\end{itemize}
%
%\begin{table*}[h!]
%  \centering
%  \caption{Research questions and their respective rationale}
%  \label{tab:table1}
%      \begin{tabular}{p{5cm}p{10cm}}
%    \toprule
%    Research questions & Rationale\\
%    \midrule
%    What is a microservice and what are its key characteristics? & This research question aims at giving an unambiguous definition of what a microservice is and charactering it. \\
%    What are the primary obstacles/challenges to the adoption of the Microservices paradigm in industry and the solutions ? & This research question aims at identifying the main hurdles that prevent practitioners from adopting Microservices and the appropriate solutions.\\
%    What are the best practices and design principles for development using Microservices and adoption of Microservices ? & This research question aims at identifying the best practice and design principles so that practitioners can be guided.\\
%    What are the aspects that researchers and practitioners should be aware? & This research question aims at highlighting the
%important publication venues of microservices
%research. It also aims for proposing a framework that covers various perspectives of Microservices. This framework (reference Figure 2 in \cite{7584353}, and the paper \cite{ZimmermannBognerSchmidtetal.2016}) will recognise and disclose the gaps in the current research hence set the direction for future research.\\    
%    \bottomrule
%  \end{tabular}
%\end{table*}

\subsection{Literature Search and Collection}

According to Vom Brocke et al.~\cite{Brocke09}, before conducting a structured literature search, it is necessary to define a research scope and provide the conceptualization of the topic. 
This has been discussed in detail in Sections~\ref{sec:scope} \emph{(assuming the current structure of the paper)}. 
Hence, the topic of concern is about vechile security ... This informs the definition of our literature search criteria.  
%Based on the research problem proposed in Section~\ref{sec:scope}, we define literature search criteria. 

We chose two popular scholarly databases, Scopus and Web of Science, for the literature search, since both databases are well-known sources of citations.\footnote{Other scholarly databases such as Proquest or EBSCO could also be used to produce a (possibly) more complete literature review. However, to keep our literature review manageable, we had to limit our search to the two databases mentioned above (Scopus and Web of Science).} 

\begin{itemize}
	\item \emph{WoS: search query}
	
	TS=(vechile security OR  xxx OR xxxx OR xxxxxx)\\
	AND LANGUAGE: (English)\\
	AND DOCUMENT TYPES: (Article OR Book OR Book Chapter OR Proceedings Paper)\\
	\emph{Timespan=2000-2018}
	
	A total of xxxxx papers were retrieved (as on xx April 2018). 
	
	\item \emph{Scopus: search query}
	
	TITLE-ABS-KEY (vechile security OR  xxx OR xxxx OR xxxxxx)\\
	AND LANGUAGE (english)\\ 
	AND DOCTYPE (ar OR ip OR bk OR ch OR cp)\\
	AND PUBYEAR $>$ 1999
		
	A total of xxxxx papers were retrieved (as on xx April 2018). 

\end{itemize}

%Finally, further filtering rules applied are:
%\footnote{In Google Scholar, some of the filtering rules, such as Language and Document types, are not supported automatically. In such case, the search results were firstly exported to Excel and then the corresponding filtering rules were applied using Excel.} 

%\medskip
%\begin{compactitem}
%	\item \emph{Language}: search papers written in English
%	\item \emph{Timespan}: search papers published between 2000 and 2017 (i.e. the most recent year of publication available)% in the database)
%	\item \emph{Document types}: search papers published as a journal article, book, book chapter, proceedings paper, and also as an article in press (Scopus only)
%	\item \emph{Subject area} (Scopus): Computer Science
%	\item \emph{Web of Science Category} (Web of Science): Computer Science Information Systems
%\end{compactitem}
%\medskip

\noindent
Next, the search results in the two databases were manually combined by removing the duplicates between the search results. 
\tablename~\ref{table:search} summarizes the literature search results. 
At the end, we obtained a total of xxx hits from our literature search.  

\begin{table}[h]
	\centering
%		\includegraphics[width=0.42\textwidth]{literature-search-results.png}
	\caption{Statistical summary of the literature search results.}
\label{table:search}
\end{table}


\subsection{Literature Selection}

Our keyword-based search criteria used were designed for a \emph{generous} coverage of representative samples of the relevant literature on the topic of microservices. 
In this second phase, we performed a careful literature selection among the overall xx hits retrieved from the previous phase. 
Our literature selection was carried out in three sequential steps.
  
Firstly, we removed papers that are obviously irrelevant, as informed by their titles, e.g.\ papers on ... 
We were cautious about excluding a paper in this step. 
A paper would not be removed unless the title indicates that it is well beyond the context of the topic on microservices.

Next, we conducted selection based on the topic of each paper. 
In this step, the abstract of a paper was studied and sometimes the content was also reviewed to gain a better understanding about the topic of the paper. 

%In addition, we also discovered and removed a number of papers that are not written in English during this step. (This usually occurs to the search results from Scopus)

Finally, we performed a paper quality screening. If a paper does not have a clear contribution and/or suffers from an unclear solution to the research question/s raised in the paper, we do not consider it qualified for review and evaluation in the next phase. A number of papers were found which suffer from quality issues and were removed. 

\tablename~\ref{table:selection} provides a summary of the number of papers excluded at each step of the literature selection phase. 
At the end, a total of xx papers were selected. 

%Based on the abstracts, we selected the papers that propose querying methods or related techniques such as indexing, caching, or query optimization. After title- and abstract-based selection, we were left with 69 papers.

\begin{table}[h]
	\centering
	%	\includegraphics[width=0.45\textwidth]{literature-selection-results.png}
	\caption{Statistical summary of the literature selection results.}
\label{table:selection}
\end{table}

The first iteration of search and selection has identified xxxx papers, and we derived a taxonomy as in Figure xxxx based on the analysis of these papers.

\subsection{Literature Analysis and Evaluation}

\begin{table*}[h]
\centering
\caption{Concept matrix - make the transition from author- to concept-centric}
\begin{tabular}{ |c|c|c|c|c| } 
\hline
Articles & \multicolumn{4}{c|}{concepts} \\
\hline
 & Vehicle Systems & Security Challenges & Existing Solutions & Prposed Framework \\ \hline
1 & \checkmark & \checkmark & & \\ 
\hline
2 & \checkmark &  & & \\ 
\hline
\end{tabular}
\end{table*}

Categorising literature selected from the above step ...


==> sec_modernVehiclesElements.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Modern Vehicle System Elements}
\label{sec:modernVehicleSystemElements}

Walk through those unique components in the modern vehicle systems, highlight their features and pave the way for the security challengs associated with these components in the next section.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sec_motivation.tex <==
\newpage

\section{Background and Motivation}
\label{sec:scope}

\begin{figure}[h!!!]
	\vspace{-.5\baselineskip}
	\begin{center}
		\includegraphics[width=1.0\linewidth]{images/taxonomy.pdf}
	\end{center}
	\vspace{-\baselineskip}
	\caption{The Taxonomy}
	\label{fig:taxonomy}
\end{figure}
